ColorGrid: A Multi-Agent Non-Stationary Environment for Goal Inference and Assistance

Autonomous agents' interactions with humans are increasingly focused on adapting to their changing preferences in order to improve assistance in real-world tasks. Effective agents must learn to accurately infer human goals, which are often hidden, to collaborate well. However, existing Multi-Agent Reinforcement Learning (MARL) environments lack the necessary attributes required to rigorously evaluate these agents' learning capabilities. To this end, we introduce ColorGrid, a novel MARL environment with customizable non-stationarity, asymmetry, and reward structure. We investigate the performance of Independent Proximal Policy Optimization (IPPO), a state-of-the-art (SOTA) MARL algorithm, in ColorGrid and find through extensive ablations that, particularly with simultaneous non-stationary and asymmetric goals between a ``leader'' agent representing a human and a ``follower'' assistant agent, ColorGrid is unsolved by IPPO. To support benchmarking future MARL algorithms, we release our environment code, model checkpoints, and trajectory visualizations at https://github.com/andreyrisukhin/ColorGrid.

==> TabsNFigs/tables/bd10_symmetric_compare_parameters.tex <==
\begin{table}[h!]
  \centering
  \small

  \caption{ ``Converged Sum Reward'' is the final net reward over 128 timesteps averaged over 16 environments. All runs use 10\% block density, non-stationary goal block color with 2\% chance of switching at each step, and \emph{symmetric} information between the leader and follower. We take the converged reward values after 80M train timesteps and average across 3 seeds (except ``0.2, None'' for which the third run crashed).}

  \begin{tabular}{l@{\hspace{0.95\tabcolsep}}
                  l@{\hspace{0.95\tabcolsep}}
                  |
                  r}
    \toprule

    \textbf{Auxiliary Loss } $\kappa$ \hspace{0.5cm} & \textbf{Penalty Annealing} \hspace{0.5cm} & \textbf{Converged Sum Reward} \\

    \midrule

    0.2 & 4M-10M & \textbf{48.8} \\

    0.2 & None & -0.7 \\

    0 & None & -1.0 \\

    0 & 4M-10M & 32.8 \\

    \bottomrule
  \end{tabular}

  \vspace{0.5cm}
  
  \label{tab:symmetric_results}
  \label{tab:training_parameters_symmetric}
\vspace{-0.5cm}
\end{table}


==> TabsNFigs/tables/env_disposition.tex <==
\begin{table}[h!]
  \centering
  \small

  \caption{ ``Converged Sum Reward'' is the final net reward over 128 timesteps averaged over 16 environments. All runs use 10\% block density, non-stationary goal block color with 2\% chance of switching at each step, and \emph{symmetric} information between the leader and follower. We take the converged reward values after 80M train timesteps and average across 3 seeds (except ``0.2, None'' for which the third run crashed).\andrey{Fix this! Incorrect label}}

  \begin{tabular}{l@{\hspace{0.95\tabcolsep}}
                  l@{\hspace{0.95\tabcolsep}}
                  |
                  r}
    \toprule

    \textbf{Goal Block Reward} \hspace{0.5cm} & \textbf{Incorrect Block Reward} \hspace{0.5cm} & \textbf{Expected Value of Random Block Collection} \\

    \midrule

    +4 & -1 &  $2/3$ \\ %$\frac{2}{3}$ \\

    +2 & -1 & $0$ \\

    +1 & -1 & $-2/3$ \\ %$-\frac{2}{3}$ \\

    % 0 & 4M-10M & 32.8 \\

    % Late & 0.2 & 4M-10M & 44.6 \\
    
    % Late & 0.2 & None & -0.9 \\

    \bottomrule
  \end{tabular}

  % TO LOOK BETTER, INCREASE THE VERTICAL SPACE BETWEEN ROWS? 
  \vspace{0.5cm}
  
  \label{tab:symmetric_results}
  \label{tab:training_parameters_symmetric}
\vspace{-0.5cm}
\end{table}


==> TabsNFigs/tables/ppo_hparams.tex <==
\begin{wraptable}{l}{0.3\textwidth}

\begin{tabular}{l c}
    \toprule
    Parameter         & Value \\
    \midrule
    LR                & 1e-4 \\
    N. Envs           & 16 \\
    N. Rollout Steps  & 128 \\
    Gamma             & 0.99 \\
    GAE Lambda        & 0.95 \\
    N. Minibatches    & 4 \\
    Update Epochs     & 4 \\
    Clip Param        & 0.2 \\
    Entropy Coef      & 0.01 \\
    Value Coef        & 0.5 \\
    Target KL         & 0.01 \\
    \bottomrule
\end{tabular}

\caption{PPO Parameters}
\label{tab:ppo_params}

\end{wraptable}
